Evaluating ChatGPT as a Recommender System: A Rigorous Approach

Large Language Models (LLMs) have recently shown impressive abilities in handling various natural language-related tasks. Among different LLMs, current studies have assessed ChatGPT's superior performance across manifold tasks, especially under the zero/few-shot prompting conditions. Given such successes, the Recommender Systems (RSs) research community have started investigating its potential applications within the recommendation scenario. However, although various methods have been proposed to integrate ChatGPT's capabilities into RSs, current research struggles to comprehensively evaluate such models while considering the peculiarities of generative models. Often, evaluations do not consider hallucinations, duplications, and out-of-the-closed domain recommendations and solely focus on accuracy metrics, neglecting the impact on beyond-accuracy facets. To bridge this gap, we propose a robust evaluation pipeline to assess ChatGPT's ability as an RS and post-process ChatGPT recommendations to account for these aspects. Through this pipeline, we investigate ChatGPT-3.5 and ChatGPT-4 performance in the recommendation task under the zero-shot condition employing the role-playing prompt. We analyze the model's functionality in three settings: the Top-N Recommendation, the cold-start recommendation, and the re-ranking of a list of recommendations, and in three domains: movies, music, and books. The experiments reveal that ChatGPT exhibits higher accuracy than the baselines on books domain. It also excels in re-ranking and cold-start scenarios while maintaining reasonable beyond-accuracy metrics. Furthermore, we measure the similarity between the ChatGPT recommendations and the other recommenders, providing insights about how ChatGPT could be categorized in the realm of recommender systems. The evaluation pipeline is publicly released for future research.

==> tables/REFERENCE.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Classic Metrics 2
\begin{table*}[t!]
\centering
\caption{Classical analysis of the baselines' results in terms of Accuracy, Diversity, Novelty, and Bias of recommendations. The arrows indicates the descending or ascending order for the best solution. Best values are in bold. Second best values are underlined.}
\label{tab:classicmetrics}

\resizebox{\textwidth}{!}{ % Resize table to fit into the text space

\begin{tabular}{clccccccccc}

\toprule

& \textbf{Model} & \textbf{nDCG} \textupfullarrow & \textbf{Recall} \textupfullarrow & \textbf{Precision} \textupfullarrow & \textbf{Gini} \textupfullarrow & \textbf{ItemCV} \textupfullarrow & \textbf{EPC} \textupfullarrow & \textbf{EFD} \textupfullarrow & \textbf{APLT} \textupfullarrow & \textbf{ARP} \textdownfullarrow \\

\midrule

\multirow{5}{*}{\adjustbox{angle=90, scale=0.8}{\textbf{Amazon Music}}}

& \easer & \textbf{0.07560} & \textbf{0.09481} & \textbf{0.02049} & 0.25846 & 8891 & \textbf{0.02863} & \textbf{0.34370} & 0.08196 & 37.6760 \\

& \user & \ul{0.07329} & \ul{0.09424} & \ul{0.02004} & 0.21426 & 8361 & \ul{0.02741} & \ul{0.32669} & 0.07363 & 42.7840 \\

& \multivae & 0.04446 & 0.06264 & 0.01269 & 0.22379 & 6556 & 0.01606 & 0.19478 & 0.05773 & 28.4834 \\

& \lightgcn & 0.06433 & 0.08632 & 0.01797 & \ul{0.33387} & \textbf{9121} & 0.02355 & 0.28666 & \ul{0.12980} & \ul{28.1607} \\

\cmidrule(lr){2-11}

& \rpb & 0.04136 & 0.05070 & 0.01071 & \textbf{0.44327} & \ul{8973} & 0.01521 & 0.20087 & \textbf{0.78420} & \textbf{4.46494} \\

% & \multicolumn{10}{l}{\vspace*{2mm}} \\ % Adjust the -2mm as needed

\midrule

\multirow{5}{*}{\adjustbox{angle=90, scale=0.8}{\textbf{Goodreads}}} 

& \easer & \textbf{0.12685} & \textbf{0.08278} & \textbf{0.09680} & 0.04144 & 6842 & \textbf{0.10599} & \textbf{1.23522} & 0.00882 & 475.874 \\

& \user & \ul{0.09842} & \ul{0.06533} & \ul{0.07416} & 0.02873 & 6434 & \ul{0.08117} & \ul{0.92929} & 0.01021 & 587.527 \\

& \multivae & 0.07090 & 0.04812 & 0.05718 & 0.05126 & 7387 & 0.05974 & 0.69948 & \ul{0.05533} & 443.142 \\

& \lightgcn & 0.06896 & 0.04835 & 0.05352 & \ul{0.06434} & \ul{7729} & 0.05722 & 0.68752 & 0.01176 & \ul{356.040} \\

& \rpb & 0.06645 & 0.04177 & 0.05066 & \textbf{0.19076} & \textbf{14941} & 0.05759 & 0.78194 & \textbf{0.71016} & \textbf{64.3545} \\

\midrule

\multirow{5}{*}{\adjustbox{angle=90, scale=0.8}{\textbf{Movielens1M}}}

& \easer & \textbf{0.36075} & \textbf{0.15574} & \textbf{0.32462} & 0.06152 & 980 & \textbf{0.27472} & \textbf{3.22977} & 0.00260 & 1198.44 \\

& \user & \ul{0.34603} & \ul{0.14980} & \ul{0.31189} & 0.04556 & 920 & 0.25320 & \ul{3.01901} & 0.00462 & 1305.30 \\

& \multivae & 0.32223 & 0.14189 & 0.29147 & \textbf{0.12550} & \textbf{1836} & \ul{0.25631} & 3.00231 & \ul{0.03657} & \ul{1002.73} \\

& \lightgcn & 0.31087 & 0.13204 & 0.28113 & \ul{0.09899} & 1481 & 0.24170 & 2.84602 & 0.02806 & 1046.17 \\

& \rpb & 0.28403 & 0.12287 & 0.27017 & 0.09266 & \ul{1588} & 0.21789 & 2.58115 & \textbf{0.17851} & \textbf{961.877} \\

\bottomrule

\end{tabular}

} % End of resizebox

\end{table*}

==> tables/_2_reranking/mostpop_rerank.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% How GPT-3.5 change in one year
\begin{table*}[t!]
\centering
\caption{\small{Analysis of ChatGPT-3.5 and ChatGPT-4 to \textbf{rerank} a list of \textbf{MostPop} items. The direction of the arrows (\textuparrow for higher, \textdownarrow for lower) denotes the preferred values for each metric. The best values are in bold. The second-best values are underlined.}}

\label{tab:mostpop_rerank}

\resizebox{\textwidth}{!}{ % Resize table to fit into the text space

\begin{tabular}{clccccccccc}

\toprule

& \textbf{Model} & \textbf{nDCG} \textupfullarrow & \textbf{Recall} \textupfullarrow & \textbf{Precision} \textupfullarrow & \textbf{Gini} \textupfullarrow & \textbf{ItemCV} \textupfullarrow & \textbf{EPC} \textupfullarrow & \textbf{EFD} \textupfullarrow & \textbf{APLT} \textupfullarrow & \textbf{ARP} \textdownfullarrow \\

\midrule

\multirow{3}{*}{\adjustbox{angle=90, scale=1}{\textbf{Books}}}

& MostPop     & 0.0009          & 0.0026          & 0.0004          & 0.0042          & 17           & 0.0002          & 0.0013          & \ul{0.3619}    & 74.8611          \\
& ChatGPT-3.5 & \ul{0.0059}    & \ul{0.0104}    & \ul{0.0028}    & \ul{0.0053}    & \textbf{52}  & \ul{0.0024}    & \ul{0.0203}    & 0.0294          & \ul{75.0315}    \\
& ChatGPT-4   & \textbf{0.0160} & \textbf{0.0249} & \textbf{0.0055} & \textbf{0.0069} & \ul{50}     & \textbf{0.0058} & \textbf{0.0508} & \textbf{0.0465} & \textbf{95.8295} \\

\midrule

\multirow{3}{*}{\adjustbox{angle=90, scale=1}{\textbf{Music}}} 

& MostPop     & 0.0800          & 0.0651          & 0.0534          & 0.0075          & 23           & 0.0491          & 0.4384          & 0.0000          & 287.7585          \\
& ChatGPT-3.5 & \ul{0.1699}    & \ul{0.1254}    & \ul{0.0971}    & \ul{0.0206}    & \textbf{239} & \ul{0.1089}    & \ul{0.9776}    & \textbf{0.0043} & \ul{262.3423}    \\
& ChatGPT-4   & \textbf{0.2071} & \textbf{0.1519} & \textbf{0.1200} & \textbf{0.0214} & \ul{58}     & \textbf{0.1341} & \textbf{1.2016} & 0.0000          & \textbf{223.1059} \\

\midrule

\multirow{3}{*}{\adjustbox{angle=90, scale=1}{\textbf{Movies}}}

& MostPop     & 0.0672          & 0.0347          & 0.0681          & 0.0061          & 26           & 0.0582          & 0.6410          & 0.0000          & \textbf{108.6320} \\
& ChatGPT-3.5 & \ul{0.1313}    & \ul{0.0703}    & \ul{0.1196}    & \textbf{0.0130} & \textbf{64}  & \ul{0.1031}    & \ul{1.1601}    & \textbf{0.0004} & \ul{148.1863}    \\
& ChatGPT-4   & \textbf{0.1681} & \textbf{0.0932} & \textbf{0.1494} & \ul{0.0112}    & \ul{44}     & \textbf{0.1275} & \textbf{1.4338} & 0.0000          & 155.4376 \\

\bottomrule

\end{tabular}

} % End of resizebox

\end{table*}

==> tables/_2_reranking/userknn_rerank.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% How GPT-3.5 change in one year
\begin{table*}[t!]
\centering
\caption{\small{Analysis of ChatGPT-3.5 and ChatGPT-4 to \textbf{rerank} a list of recommendations provided by \textbf{Nearest Neighbors}. The direction of the arrows (\textuparrow for higher, \textdownarrow for lower) denotes the preferred values for each metric. The best values are in bold. The second-best values are underlined.}}

\label{tab:userknn_rerank}

\resizebox{\textwidth}{!}{ % Resize table to fit into the text space

\begin{tabular}{clccccccccc}

\toprule

& \textbf{Model} & \textbf{nDCG} \textupfullarrow & \textbf{Recall} \textupfullarrow & \textbf{Precision} \textupfullarrow & \textbf{Gini} \textupfullarrow & \textbf{ItemCV} \textupfullarrow & \textbf{EPC} \textupfullarrow & \textbf{EFD} \textupfullarrow & \textbf{APLT} \textupfullarrow & \textbf{ARP} \textdownfullarrow \\

\midrule

\multirow{3}{*}{\adjustbox{angle=90, scale=1}{\textbf{Books}}}

& Nearest Neighbors & 0.0149          & 0.0253          & 0.0055          & \textbf{0.2654} & \textbf{1608} & 0.0055          & 0.0518          & \textbf{0.1788} & \textbf{36.1033} \\
& ChatGPT-3.5       & \ul{0.0292}    & \ul{0.0375}    & \ul{0.0081}    & \ul{0.1415}    & \ul{1243}    & \ul{0.0109}    & \ul{0.1007}    & \ul{0.1031}    & \ul{52.1764}    \\
& ChatGPT-4         & \textbf{0.0451} & \textbf{0.0620} & \textbf{0.0138} & 0.0677          & 719           & \textbf{0.0168} & \textbf{0.1537} & 0.0450          & 73.2015 \\

\midrule

\multirow{3}{*}{\adjustbox{angle=90, scale=1}{\textbf{Music}}} 

& Nearest Neighbors & 0.0533          & 0.0699          & 0.0520          & \textbf{0.4212} & \textbf{1402} & 0.0481          & 0.4701          & \textbf{0.1947} & \textbf{87.8391} \\
& ChatGPT-3.5       & \ul{0.2019}    & \ul{0.1670}    & \ul{0.1222}    & \ul{0.2395}    & \ul{1145}    & \ul{0.1362}    & \ul{1.2965}    & \ul{0.1023}    & \ul{124.7856}   \\
& ChatGPT-4         & \textbf{0.2653} & \textbf{0.2171} & \textbf{0.1592} & 0.1652          & 865           & \textbf{0.1749} & \textbf{1.6649} & 0.0697          & 134.0541 \\

\midrule

\multirow{3}{*}{\adjustbox{angle=90, scale=1}{\textbf{Movies}}}

& Nearest Neighbors & 0.0859          & 0.0701          & 0.1008          & \textbf{0.2818} & \textbf{1149} & 0.0845          & 0.9223          & \textbf{0.1388} & \textbf{66.6738} \\
& ChatGPT-3.5       & \ul{0.1732}    & \ul{0.1098}    & \ul{0.1594}    & \ul{0.0909}    & \ul{640}     & \ul{0.1400}    & \ul{1.5521}    & \ul{0.0328}    & 111.8979         \\
& ChatGPT-4         & \textbf{0.2283} & \textbf{0.1405} & \textbf{0.2030} & 0.0558          & 419           & \textbf{0.1778} & \textbf{1.9653} & 0.0127          & \ul{123.6421} \\

\bottomrule

\end{tabular}

} % End of resizebox

\end{table*}

==> tests/kivat_table.tex <==
\begin{tikzpicture}
\tkzKiviatDiagramFromFile[
        scale=.5,
        label distance=.5cm,
        gap     = 1,label space=3,  
        lattice = 10]{tableae.dat}
\tkzKiviatLineFromFile[thick,
                       color      = blue,
                       mark       = ball,
                       ball color = blue,
                       mark size  = 4pt,
                       fill       = blue!20]{tableae.dat}{2}
\tkzKiviatLineFromFile[thick,
                       color      = red,
                       mark       = ball,
                       ball color = red,
                       mark size  = 4pt,
                       fill       = red!20]{tableae.dat}{1} 
\end{tikzpicture}
